InstantEdit: Text-Guided Few-Step Image Editing with Piecewise Rectified Flow

We propose a fast text-guided image editing method called InstantEdit based on the RectifiedFlow framework, which is structured as a few-step editing process that preserves critical content while following closely to textual instructions. Our approach leverages the straight sampling trajectories of RectifiedFlow by introducing a specialized inversion strategy called PerRFI. To maintain consistent while editable results for RectifiedFlow model, we further propose a novel regeneration method, Inversion Latent Injection, which effectively reuses latent information obtained during inversion to facilitate more coherent and detailed regeneration. Additionally, we propose a Disentangled Prompt Guidance technique to balance editability with detail preservation, and integrate a Canny-conditioned ControlNet to incorporate structural cues and suppress artifacts. Evaluation on the PIE image editing dataset demonstrates that InstantEdit is not only fast but also achieves better qualitative and quantitative results compared to state-of-the-art few-step editing methods.

==> figs/latex/supp_diverse_edit.tex <==
\begin{figure*}[h]
 \centering
 \begin{minipage}{\textwidth}
\includegraphics[width=\linewidth]{figs/supp_diverse_edit.pdf}
\caption{ Additional editing results with diverse text prompts.
\label{fig:supp_diver_edit}
}
\end{minipage}
\end{figure*}
